Improved Discrete RRT for Coordinated Multi-robot Planning

This paper addresses the problem of coordination of a fleet of mobile robots - the problem of finding an optimal set of collision-free trajectories for individual robots in the fleet. Many approaches have been introduced during the last decades, but a minority of them is practically applicable, i.e. fast, producing near-optimal solutions, and complete. We propose a novel probabilistic approach based on the Rapidly Exploring Random Tree algorithm (RRT) by significantly improving its multi-robot variant for discrete environments. The presented experimental results show that the proposed approach is fast enough to solve problems with tens of robots in seconds. Although the solutions generated by the approach are slightly worse than one of the best state-of-the-art algorithms presented in (ter Mors et al., 2010), it solves problems where ter Mors's algorithm fails.

==> sota.tex <==
\section{Introduction/State of the Art}

Multi-robot path planning and motion coordination has been studied since 1980s and many techniques have
been developed during this period, see [1] for a nice overview. This problem (formulated as the warehouseman’s
problem) was proved to be PSPACE-complete [2]. For the case where robots move on a predefined graph (like
in SafeLog) complexity of the problem can be reduced, nevertheless it is still NP-hard [3], which means that
optimal solutions cannot be generally found in a reasonable time for non-trivial instances (e.g., for a number of
robots in order of tens).
Solutions to the problem consider either coupled or decoupled approaches. Centralized (coupled) approaches
consider the multi-robot team as a multi-body robot for which classical single-robot path planning can be applied
in a composite configuration space. Traditional centralized methods are based on complete (i.e., the algorithm finds
a solution if it exists or reports that no solution exists otherwise) and optimal classical algorithms and provide
optimal solutions [4], [5], [6]. However, these approaches require computational time exponential in the dimension
of the composite configuration space so they are appropriate for small-sized problems only. This drawback lead
to development of methods that prune the search space. For instance, Berg et al. [7] decompose any instance
of the problem into a sequence of sub-problems where each subproblem can be solved independently from the
others. The Biased Cost Pathfinding [8] employs generalised central decision maker that resolves collision points
on paths that were pre-computed independently per unit, by replanning colliding units around a highest priority
unit. Another approach is to design an algorithm based on a specific topology describing the environment.
Peasgood [9] presents a multi-phase approach with linear time complexity based on searching a minimum
spanning tree of the graph, while an approach for grid-like environments is introduced in [10]. A flow-annotated
search graph inspired by two-way roads is built to avoid head-to-head collisions and to reduce the branching
factor in search. Nevertheless, the computational complexity is still high (e.g., [7] solves a problem with 40 robots
in 12 minutes, [10] needs approx. 30 seconds for 400 robots).
On the contrary, decoupled methods present a coordination phase separated from the path planning phase.
These approaches provide solutions typically in orders of magnitude faster times than coupled planners, but
these solutions are sub-optimal. Moreover, the decoupled methods are often not complete as they may suffer
from deadlocks. These approaches are divided into two categories: path coordination techniques and prioritized
planning. Path coordination considers tuning the velocities of robots along the precomputed trajectories to avoid
collisions [11], [12], while prioritized planning computes trajectories sequentially for the particular robots based
on the robots’ priorities. Robots with already determined trajectories are considered as moving obstacles to be
avoided by robots with lower priorities [13], [14], [15].
Several computationally efficient heuristics have been introduced recently enabling to solve problems for tens
of robots in seconds. Windowed Hierarchical Cooperative A* algorithm (WHCA*) employs heuristic search in
a space-time domain based on hierarchical A* limited to a fixed depth [16]. Chiew [17] proposes an algorithm
for n
2 vehicles on a n × n mesh topology of path network allowing simultaneous movement of vehicles in a
corridor in opposite directions (which is not possible in the SafeLog scenario) with computational complexity
O(n
2
). Luna and Bekros [18] present and complete heuristics for general problems with at most n − 2 robots
in a graph with n vertices based on combination on two primitives - "push" forces robots towards a specific
path, while "swap" switches positions of two robots if they are to be colliding. An extension which divides the
graph into subgraphs within which it is possible for agents to reach any position of the subgraph, and then uses
"push", "swap", and "rotate" operations is presented in [19]. Wang and Botea [20] identifie classes of multi-robot
path planning problems that can be solved in polynomial time (Slidable) and introduces an algorithm with low
polynomial upper bounds for time, space and solution length. Finally, Wang and Wooi [21] formulate multi-robot
path planning as an optimization problem and approximate the objective function by adopting a maximum
entropy function, which is minimized by a probabilistic iterative algorithm
